Deep Value Benchmark: Measuring Whether Models Generalize Deep Values or Shallow Preferences

We introduce the Deep Value Benchmark (DVB), an evaluation framework that directly tests whether large language models (LLMs) learn fundamental human values or merely surface-level preferences. This distinction is critical for AI alignment: Systems that capture deeper values are likely to generalize human intentions robustly, while those that capture only superficial patterns in preference data risk producing misaligned behavior. The DVB uses a novel experimental design with controlled confounding between deep values (e.g., moral principles) and shallow features (e.g., superficial attributes). In the training phase, we expose LLMs to human preference data with deliberately correlated deep and shallow features -- for instance, where a user consistently prefers (non-maleficence, formal language) options over (justice, informal language) alternatives. The testing phase then breaks these correlations, presenting choices between (justice, formal language) and (non-maleficence, informal language) options. This design allows us to precisely measure a model's Deep Value Generalization Rate (DVGR) -- the probability of generalizing based on the underlying value rather than the shallow feature. Across 9 different models, the average DVGR is just 0.30. All models generalize deep values less than chance. Larger models have a (slightly) lower DVGR than smaller models. We are releasing our dataset, which was subject to three separate human validation experiments. DVB provides an interpretable measure of a core feature of alignment.

==> tables/work_acts.tex <==
\begin{longtable}{ll}
\caption{Clusters and top 10 work activities of associated ONET occuptations.} \label{work_acts} \\
\toprule
 & item_name \\
cluster &  \\
\midrule
\endfirsthead
\caption[]{Clusters and top 10 work activities of associated ONET occuptations.} \\
\toprule
 & item_name \\
cluster &  \\
\midrule
\endhead
\midrule
\multicolumn{2}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
commerce & Establishing and Maintaining Interpersonal Relationships,Getting Information,Communicating with Supervisors, Peers, or Subordinates,Organizing, Planning, and Prioritizing Work,Making Decisions and Solving Problems,Updating and Using Relevant Knowledge,Communicating with People Outside the Organization,Processing Information,Working with Computers,Analyzing Data or Information,Identifying Objects, Actions, and Events,Resolving Conflicts and Negotiating with Others,Evaluating Information to Determine Compliance with Standards,Thinking Creatively,Documenting/Recording Information,Scheduling Work and Activities,Monitoring Processes, Materials, or Surroundings,Coordinating the Work and Activities of Others,Judging the Qualities of Objects, Services, or People,Providing Consultation and Advice to Others,Developing Objectives and Strategies,Coaching and Developing Others,Selling or Influencing Others,Interpreting the Meaning of Information for Others,Training and Teaching Others,Performing Administrative Activities,Developing and Building Teams,Guiding, Directing, and Motivating Subordinates,Performing for or Working Directly with the Public,Monitoring and Controlling Resources,Estimating the Quantifiable Characteristics of Products, Events, or Information,Assisting and Caring for Others,Staffing Organizational Units,Inspecting Equipment, Structures, or Materials,Handling and Moving Objects,Performing General Physical Activities,Controlling Machines and Processes,Operating Vehicles, Mechanized Devices, or Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment,Repairing and Maintaining Electronic Equipment,Repairing and Maintaining Mechanical Equipment \\
communication & Updating and Using Relevant Knowledge,Getting Information,Thinking Creatively,Communicating with Supervisors, Peers, or Subordinates,Making Decisions and Solving Problems,Working with Computers,Organizing, Planning, and Prioritizing Work,Establishing and Maintaining Interpersonal Relationships,Processing Information,Identifying Objects, Actions, and Events,Analyzing Data or Information,Communicating with People Outside the Organization,Documenting/Recording Information,Interpreting the Meaning of Information for Others,Monitoring Processes, Materials, or Surroundings,Scheduling Work and Activities,Providing Consultation and Advice to Others,Evaluating Information to Determine Compliance with Standards,Developing Objectives and Strategies,Judging the Qualities of Objects, Services, or People,Coordinating the Work and Activities of Others,Training and Teaching Others,Coaching and Developing Others,Resolving Conflicts and Negotiating with Others,Developing and Building Teams,Estimating the Quantifiable Characteristics of Products, Events, or Information,Guiding, Directing, and Motivating Subordinates,Performing Administrative Activities,Selling or Influencing Others,Monitoring and Controlling Resources,Performing for or Working Directly with the Public,Inspecting Equipment, Structures, or Materials,Assisting and Caring for Others,Handling and Moving Objects,Staffing Organizational Units,Performing General Physical Activities,Controlling Machines and Processes,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment,Repairing and Maintaining Electronic Equipment,Repairing and Maintaining Mechanical Equipment,Operating Vehicles, Mechanized Devices, or Equipment \\
customer_service & Establishing and Maintaining Interpersonal Relationships,Getting Information,Communicating with Supervisors, Peers, or Subordinates,Organizing, Planning, and Prioritizing Work,Updating and Using Relevant Knowledge,Making Decisions and Solving Problems,Working with Computers,Processing Information,Communicating with People Outside the Organization,Performing for or Working Directly with the Public,Identifying Objects, Actions, and Events,Documenting/Recording Information,Resolving Conflicts and Negotiating with Others,Evaluating Information to Determine Compliance with Standards,Monitoring Processes, Materials, or Surroundings,Analyzing Data or Information,Performing Administrative Activities,Thinking Creatively,Selling or Influencing Others,Scheduling Work and Activities,Judging the Qualities of Objects, Services, or People,Interpreting the Meaning of Information for Others,Training and Teaching Others,Coordinating the Work and Activities of Others,Coaching and Developing Others,Developing Objectives and Strategies,Assisting and Caring for Others,Providing Consultation and Advice to Others,Developing and Building Teams,Estimating the Quantifiable Characteristics of Products, Events, or Information,Handling and Moving Objects,Guiding, Directing, and Motivating Subordinates,Performing General Physical Activities,Monitoring and Controlling Resources,Inspecting Equipment, Structures, or Materials,Controlling Machines and Processes,Staffing Organizational Units,Operating Vehicles, Mechanized Devices, or Equipment,Repairing and Maintaining Electronic Equipment,Repairing and Maintaining Mechanical Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment \\
education & Training and Teaching Others,Updating and Using Relevant Knowledge,Organizing, Planning, and Prioritizing Work,Getting Information,Thinking Creatively,Establishing and Maintaining Interpersonal Relationships,Communicating with Supervisors, Peers, or Subordinates,Making Decisions and Solving Problems,Interpreting the Meaning of Information for Others,Coaching and Developing Others,Identifying Objects, Actions, and Events,Processing Information,Analyzing Data or Information,Working with Computers,Developing Objectives and Strategies,Documenting/Recording Information,Scheduling Work and Activities,Judging the Qualities of Objects, Services, or People,Communicating with People Outside the Organization,Monitoring Processes, Materials, or Surroundings,Providing Consultation and Advice to Others,Coordinating the Work and Activities of Others,Performing for or Working Directly with the Public,Evaluating Information to Determine Compliance with Standards,Resolving Conflicts and Negotiating with Others,Guiding, Directing, and Motivating Subordinates,Assisting and Caring for Others,Developing and Building Teams,Performing Administrative Activities,Estimating the Quantifiable Characteristics of Products, Events, or Information,Monitoring and Controlling Resources,Handling and Moving Objects,Selling or Influencing Others,Inspecting Equipment, Structures, or Materials,Performing General Physical Activities,Staffing Organizational Units,Controlling Machines and Processes,Repairing and Maintaining Electronic Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment,Operating Vehicles, Mechanized Devices, or Equipment,Repairing and Maintaining Mechanical Equipment \\
finance & Communicating with Supervisors, Peers, or Subordinates,Getting Information,Making Decisions and Solving Problems,Establishing and Maintaining Interpersonal Relationships,Organizing, Planning, and Prioritizing Work,Updating and Using Relevant Knowledge,Processing Information,Analyzing Data or Information,Communicating with People Outside the Organization,Working with Computers,Identifying Objects, Actions, and Events,Evaluating Information to Determine Compliance with Standards,Resolving Conflicts and Negotiating with Others,Documenting/Recording Information,Scheduling Work and Activities,Thinking Creatively,Coordinating the Work and Activities of Others,Providing Consultation and Advice to Others,Developing Objectives and Strategies,Coaching and Developing Others,Monitoring Processes, Materials, or Surroundings,Interpreting the Meaning of Information for Others,Judging the Qualities of Objects, Services, or People,Developing and Building Teams,Guiding, Directing, and Motivating Subordinates,Training and Teaching Others,Performing Administrative Activities,Monitoring and Controlling Resources,Estimating the Quantifiable Characteristics of Products, Events, or Information,Selling or Influencing Others,Performing for or Working Directly with the Public,Staffing Organizational Units,Assisting and Caring for Others,Inspecting Equipment, Structures, or Materials,Performing General Physical Activities,Handling and Moving Objects,Controlling Machines and Processes,Operating Vehicles, Mechanized Devices, or Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment,Repairing and Maintaining Electronic Equipment,Repairing and Maintaining Mechanical Equipment \\
healthcare & Assisting and Caring for Others,Updating and Using Relevant Knowledge,Getting Information,Identifying Objects, Actions, and Events,Establishing and Maintaining Interpersonal Relationships,Documenting/Recording Information,Making Decisions and Solving Problems,Communicating with Supervisors, Peers, or Subordinates,Monitoring Processes, Materials, or Surroundings,Organizing, Planning, and Prioritizing Work,Processing Information,Evaluating Information to Determine Compliance with Standards,Performing for or Working Directly with the Public,Training and Teaching Others,Working with Computers,Handling and Moving Objects,Interpreting the Meaning of Information for Others,Analyzing Data or Information,Judging the Qualities of Objects, Services, or People,Thinking Creatively,Inspecting Equipment, Structures, or Materials,Resolving Conflicts and Negotiating with Others,Coaching and Developing Others,Performing General Physical Activities,Scheduling Work and Activities,Communicating with People Outside the Organization,Coordinating the Work and Activities of Others,Developing and Building Teams,Developing Objectives and Strategies,Providing Consultation and Advice to Others,Guiding, Directing, and Motivating Subordinates,Estimating the Quantifiable Characteristics of Products, Events, or Information,Performing Administrative Activities,Controlling Machines and Processes,Monitoring and Controlling Resources,Selling or Influencing Others,Staffing Organizational Units,Repairing and Maintaining Electronic Equipment,Repairing and Maintaining Mechanical Equipment,Operating Vehicles, Mechanized Devices, or Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment \\
hr & Getting Information,Making Decisions and Solving Problems,Communicating with Supervisors, Peers, or Subordinates,Establishing and Maintaining Interpersonal Relationships,Organizing, Planning, and Prioritizing Work,Processing Information,Updating and Using Relevant Knowledge,Analyzing Data or Information,Communicating with People Outside the Organization,Working with Computers,Evaluating Information to Determine Compliance with Standards,Identifying Objects, Actions, and Events,Documenting/Recording Information,Resolving Conflicts and Negotiating with Others,Interpreting the Meaning of Information for Others,Providing Consultation and Advice to Others,Thinking Creatively,Developing Objectives and Strategies,Scheduling Work and Activities,Performing Administrative Activities,Monitoring Processes, Materials, or Surroundings,Judging the Qualities of Objects, Services, or People,Training and Teaching Others,Coaching and Developing Others,Coordinating the Work and Activities of Others,Developing and Building Teams,Guiding, Directing, and Motivating Subordinates,Estimating the Quantifiable Characteristics of Products, Events, or Information,Selling or Influencing Others,Performing for or Working Directly with the Public,Monitoring and Controlling Resources,Assisting and Caring for Others,Staffing Organizational Units,Inspecting Equipment, Structures, or Materials,Performing General Physical Activities,Handling and Moving Objects,Controlling Machines and Processes,Operating Vehicles, Mechanized Devices, or Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment,Repairing and Maintaining Electronic Equipment,Repairing and Maintaining Mechanical Equipment \\
legal & Getting Information,Making Decisions and Solving Problems,Evaluating Information to Determine Compliance with Standards,Processing Information,Updating and Using Relevant Knowledge,Analyzing Data or Information,Identifying Objects, Actions, and Events,Organizing, Planning, and Prioritizing Work,Communicating with Supervisors, Peers, or Subordinates,Establishing and Maintaining Interpersonal Relationships,Interpreting the Meaning of Information for Others,Resolving Conflicts and Negotiating with Others,Documenting/Recording Information,Working with Computers,Communicating with People Outside the Organization,Judging the Qualities of Objects, Services, or People,Thinking Creatively,Performing Administrative Activities,Performing for or Working Directly with the Public,Scheduling Work and Activities,Monitoring Processes, Materials, or Surroundings,Providing Consultation and Advice to Others,Developing Objectives and Strategies,Coordinating the Work and Activities of Others,Training and Teaching Others,Coaching and Developing Others,Estimating the Quantifiable Characteristics of Products, Events, or Information,Assisting and Caring for Others,Developing and Building Teams,Selling or Influencing Others,Guiding, Directing, and Motivating Subordinates,Monitoring and Controlling Resources,Handling and Moving Objects,Controlling Machines and Processes,Inspecting Equipment, Structures, or Materials,Staffing Organizational Units,Performing General Physical Activities,Operating Vehicles, Mechanized Devices, or Equipment,Repairing and Maintaining Electronic Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment,Repairing and Maintaining Mechanical Equipment \\
productivity & Working with Computers,Getting Information,Processing Information,Communicating with Supervisors, Peers, or Subordinates,Updating and Using Relevant Knowledge,Making Decisions and Solving Problems,Organizing, Planning, and Prioritizing Work,Establishing and Maintaining Interpersonal Relationships,Analyzing Data or Information,Identifying Objects, Actions, and Events,Documenting/Recording Information,Evaluating Information to Determine Compliance with Standards,Thinking Creatively,Interpreting the Meaning of Information for Others,Monitoring Processes, Materials, or Surroundings,Communicating with People Outside the Organization,Scheduling Work and Activities,Resolving Conflicts and Negotiating with Others,Judging the Qualities of Objects, Services, or People,Providing Consultation and Advice to Others,Training and Teaching Others,Developing Objectives and Strategies,Coordinating the Work and Activities of Others,Performing Administrative Activities,Estimating the Quantifiable Characteristics of Products, Events, or Information,Coaching and Developing Others,Developing and Building Teams,Guiding, Directing, and Motivating Subordinates,Monitoring and Controlling Resources,Performing for or Working Directly with the Public,Assisting and Caring for Others,Inspecting Equipment, Structures, or Materials,Selling or Influencing Others,Handling and Moving Objects,Staffing Organizational Units,Controlling Machines and Processes,Performing General Physical Activities,Repairing and Maintaining Electronic Equipment,Drafting, Laying Out, and Specifying Technical Devices, Parts, and Equipment,Operating Vehicles, Mechanized Devices, or Equipment,Repairing and Maintaining Mechanical Equipment \\
\end{longtable}

